Dealing with Distribution Mismatch in Semi-supervised Deep Learning for Covid-19 Detection Using Chest X-ray Images: A Novel Approach Using Feature Densities

In the context of the global coronavirus pandemic, different deep learning solutions for infected subject detection using chest X-ray images have been proposed. However, deep learning models usually need large labelled datasets to be effective. Semi-supervised deep learning is an attractive alternative, where unlabelled data is leveraged to improve the overall model's accuracy. However, in real-world usage settings, an unlabelled dataset might present a different distribution than the labelled dataset (i.e. the labelled dataset was sampled from a target clinic and the unlabelled dataset from a source clinic). This results in a distribution mismatch between the unlabelled and labelled datasets. In this work, we assess the impact of the distribution mismatch between the labelled and the unlabelled datasets, for a semi-supervised model trained with chest X-ray images, for COVID-19 detection. Under strong distribution mismatch conditions, we found an accuracy hit of almost 30\%, suggesting that the unlabelled dataset distribution has a strong influence in the behaviour of the model. Therefore, we propose a straightforward approach to diminish the impact of such distribution mismatch. Our proposed method uses a density approximation of the feature space. It is built upon the target dataset to filter out the observations in the source unlabelled dataset that might harm the accuracy of the semi-supervised model. It assumes that a small labelled source dataset is available together with a larger source unlabelled dataset. Our proposed method does not require any model training, it is simple and computationally cheap. We compare our proposed method against two popular state of the art out-of-distribution data detectors, which are also cheap and simple to implement. In our tests, our method yielded accuracy gains of up to 32\%, when compared to the previous state of the art methods.

==> images/deltas_gammas.tex <==
\begingroup 
\makeatletter 
\begin{pgfpicture} 
\pgfpathrectangle{\pgfpointorigin}{\pgfqpoint{6.400000in}{4.800000in}} 
\pgfusepath{use as bounding box, clip} 
\begin{pgfscope} 
\pgfsetbuttcap 
\pgfsetmiterjoin 
\definecolor{currentfill}{rgb}{1.000000,1.000000,1.000000} 
\pgfsetfillcolor{currentfill} 
\pgfsetlinewidth{0.000000pt} 
\definecolor{currentstroke}{rgb}{1.000000,1.000000,1.000000} 
\pgfsetstrokecolor{currentstroke} 
\pgfsetdash{}{0pt} 
\pgfpathmoveto{\pgfqpoint{0.000000in}{0.000000in}} 
\pgfpathlineto{\pgfqpoint{6.400000in}{0.000000in}} 
\pgfpathlineto{\pgfqpoint{6.400000in}{4.800000in}} 
\pgfpathlineto{\pgfqpoint{0.000000in}{4.800000in}} 
\pgfpathclose 
\pgfusepath{fill} 
\end{pgfscope} 
\begin{pgfscope} 
\pgfsetbuttcap 
\pgfsetmiterjoin 
\definecolor{currentfill}{rgb}{1.000000,1.000000,1.000000} 
\pgfsetfillcolor{currentfill} 
\pgfsetlinewidth{0.000000pt} 
\definecolor{currentstroke}{rgb}{0.000000,0.000000,0.000000} 
\pgfsetstrokecolor{currentstroke} 
\pgfsetstrokeopacity{0.000000} 
\pgfsetdash{}{0pt} 
\pgfpathmoveto{\pgfqpoint{0.800000in}{0.528000in}} 
\pgfpathlineto{\pgfqpoint{5.760000in}{0.528000in}} 
\pgfpathlineto{\pgfqpoint{5.760000in}{4.224000in}} 
\pgfpathlineto{\pgfqpoint{0.800000in}{4.224000in}} 
\pgfpathclose 
\pgfusepath{fill} 
\end{pgfscope} 
\begin{pgfscope} 
\pgfsetbuttcap 
\pgfsetroundjoin 
\definecolor{currentfill}{rgb}{0.000000,0.000000,0.000000} 
\pgfsetfillcolor{currentfill} 
\pgfsetlinewidth{0.803000pt} 
\definecolor{currentstroke}{rgb}{0.000000,0.000000,0.000000} 
\pgfsetstrokecolor{currentstroke} 
\pgfsetdash{}{0pt} 
\pgfsys@defobject{currentmarker}{\pgfqpoint{0.000000in}{-0.048611in}}{\pgfqpoint{0.000000in}{0.000000in}}{ 
\pgfpathmoveto{\pgfqpoint{0.000000in}{0.000000in}} 
\pgfpathlineto{\pgfqpoint{0.000000in}{-0.048611in}} 
\pgfusepath{stroke,fill} 
} 
\begin{pgfscope} 
\pgfsys@transformshift{1.078521in}{0.528000in} 
\pgfsys@useobject{currentmarker}{} 
\end{pgfscope} 
\end{pgfscope} 
\begin{pgfscope} 
\definecolor{textcolor}{rgb}{0.000000,0.000000,0.000000} 
\pgfsetstrokecolor{textcolor} 
\pgfsetfillcolor{textcolor} 
\pgftext[x=1.078521in,y=0.430778in,,top]{\color{textcolor}\rmfamily\fontsize{20.000000}{24.000000}\selectfont \(\displaystyle 1100\)} 
\end{pgfscope} 
\begin{pgfscope} 
\pgfsetbuttcap 
\pgfsetroundjoin 
\definecolor{currentfill}{rgb}{0.000000,0.000000,0.000000} 
\pgfsetfillcolor{currentfill} 
\pgfsetlinewidth{0.803000pt} 
\definecolor{currentstroke}{rgb}{0.000000,0.000000,0.000000} 
\pgfsetstrokecolor{currentstroke} 
\pgfsetdash{}{0pt} 
\pgfsys@defobject{currentmarker}{\pgfqpoint{0.000000in}{-0.048611in}}{\pgfqpoint{0.000000in}{0.000000in}}{ 
\pgfpathmoveto{\pgfqpoint{0.000000in}{0.000000in}} 
\pgfpathlineto{\pgfqpoint{0.000000in}{-0.048611in}} 
\pgfusepath{stroke,fill} 
} 
\begin{pgfscope} 
\pgfsys@transformshift{2.959027in}{0.528000in} 
\pgfsys@useobject{currentmarker}{} 
\end{pgfscope} 
\end{pgfscope} 
\begin{pgfscope} 
\definecolor{textcolor}{rgb}{0.000000,0.000000,0.000000} 
\pgfsetstrokecolor{textcolor} 
\pgfsetfillcolor{textcolor} 
\pgftext[x=2.959027in,y=0.430778in,,top]{\color{textcolor}\rmfamily\fontsize{20.000000}{24.000000}\selectfont \(\displaystyle 1200\)} 
\end{pgfscope} 
\begin{pgfscope} 
\pgfsetbuttcap 
\pgfsetroundjoin 
\definecolor{currentfill}{rgb}{0.000000,0.000000,0.000000} 
\pgfsetfillcolor{currentfill} 
\pgfsetlinewidth{0.803000pt} 
\definecolor{currentstroke}{rgb}{0.000000,0.000000,0.000000} 
\pgfsetstrokecolor{currentstroke} 
\pgfsetdash{}{0pt} 
\pgfsys@defobject{currentmarker}{\pgfqpoint{0.000000in}{-0.048611in}}{\pgfqpoint{0.000000in}{0.000000in}}{ 
\pgfpathmoveto{\pgfqpoint{0.000000in}{0.000000in}} 
\pgfpathlineto{\pgfqpoint{0.000000in}{-0.048611in}} 
\pgfusepath{stroke,fill} 
} 
\begin{pgfscope} 
\pgfsys@transformshift{4.839534in}{0.528000in} 
\pgfsys@useobject{currentmarker}{} 
\end{pgfscope} 
\end{pgfscope} 
\begin{pgfscope} 
\definecolor{textcolor}{rgb}{0.000000,0.000000,0.000000} 
\pgfsetstrokecolor{textcolor} 
\pgfsetfillcolor{textcolor} 
\pgftext[x=4.839534in,y=0.430778in,,top]{\color{textcolor}\rmfamily\fontsize{20.000000}{24.000000}\selectfont \(\displaystyle 1300\)} 
\end{pgfscope} 
\begin{pgfscope} 
\definecolor{textcolor}{rgb}{0.000000,0.000000,0.000000} 
\pgfsetstrokecolor{textcolor} 
\pgfsetfillcolor{textcolor} 
\pgftext[x=3.280000in,y=0.119155in,,top]{\color{textcolor}\rmfamily\fontsize{20.000000}{24.000000}\selectfont Feature values} 
\end{pgfscope} 
\begin{pgfscope} 
\pgfsetbuttcap 
\pgfsetroundjoin 
\definecolor{currentfill}{rgb}{0.000000,0.000000,0.000000} 
\pgfsetfillcolor{currentfill} 
\pgfsetlinewidth{0.803000pt} 
\definecolor{currentstroke}{rgb}{0.000000,0.000000,0.000000} 
\pgfsetstrokecolor{currentstroke} 
\pgfsetdash{}{0pt} 
\pgfsys@defobject{currentmarker}{\pgfqpoint{-0.048611in}{0.000000in}}{\pgfqpoint{0.000000in}{0.000000in}}{ 
\pgfpathmoveto{\pgfqpoint{0.000000in}{0.000000in}} 
\pgfpathlineto{\pgfqpoint{-0.048611in}{0.000000in}} 
\pgfusepath{stroke,fill} 
} 
\begin{pgfscope} 
\pgfsys@transformshift{0.800000in}{0.696000in} 
\pgfsys@useobject{currentmarker}{} 
\end{pgfscope} 
\end{pgfscope} 
\begin{pgfscope} 
\definecolor{textcolor}{rgb}{0.000000,0.000000,0.000000} 
\pgfsetstrokecolor{textcolor} 
\pgfsetfillcolor{textcolor} 
\pgftext[x=0.360215in,y=0.595981in,left,base]{\color{textcolor}\rmfamily\fontsize{20.000000}{24.000000}\selectfont \(\displaystyle 0.0\)} 
\end{pgfscope} 
\begin{pgfscope} 
\pgfsetbuttcap 
\pgfsetroundjoin 
\definecolor{currentfill}{rgb}{0.000000,0.000000,0.000000} 
\pgfsetfillcolor{currentfill} 
\pgfsetlinewidth{0.803000pt} 
\definecolor{currentstroke}{rgb}{0.000000,0.000000,0.000000} 
\pgfsetstrokecolor{currentstroke} 
\pgfsetdash{}{0pt} 
\pgfsys@defobject{currentmarker}{\pgfqpoint{-0.048611in}{0.000000in}}{\pgfqpoint{0.000000in}{0.000000in}}{ 
\pgfpathmoveto{\pgfqpoint{0.000000in}{0.000000in}} 
\pgfpathlineto{\pgfqpoint{-0.048611in}{0.000000in}} 
\pgfusepath{stroke,fill} 
} 
\begin{pgfscope} 
\pgfsys@transformshift{0.800000in}{1.816000in} 
\pgfsys@useobject{currentmarker}{} 
\end{pgfscope} 
\end{pgfscope} 
\begin{pgfscope} 
\definecolor{textcolor}{rgb}{0.000000,0.000000,0.000000} 
\pgfsetstrokecolor{textcolor} 
\pgfsetfillcolor{textcolor} 
\pgftext[x=0.360215in,y=1.715981in,left,base]{\color{textcolor}\rmfamily\fontsize{20.000000}{24.000000}\selectfont \(\displaystyle 0.2\)} 
\end{pgfscope} 
\begin{pgfscope} 
\pgfsetbuttcap 
\pgfsetroundjoin 
\definecolor{currentfill}{rgb}{0.000000,0.000000,0.000000} 
\pgfsetfillcolor{currentfill} 
\pgfsetlinewidth{0.803000pt} 
\definecolor{currentstroke}{rgb}{0.000000,0.000000,0.000000} 
\pgfsetstrokecolor{currentstroke} 
\pgfsetdash{}{0pt} 
\pgfsys@defobject{currentmarker}{\pgfqpoint{-0.048611in}{0.000000in}}{\pgfqpoint{0.000000in}{0.000000in}}{ 
\pgfpathmoveto{\pgfqpoint{0.000000in}{0.000000in}} 
\pgfpathlineto{\pgfqpoint{-0.048611in}{0.000000in}} 
\pgfusepath{stroke,fill} 
} 
\begin{pgfscope} 
\pgfsys@transformshift{0.800000in}{2.936000in} 
\pgfsys@useobject{currentmarker}{} 
\end{pgfscope} 
\end{pgfscope} 
\begin{pgfscope} 
\definecolor{textcolor}{rgb}{0.000000,0.000000,0.000000} 
\pgfsetstrokecolor{textcolor} 
\pgfsetfillcolor{textcolor} 
\pgftext[x=0.360215in,y=2.835981in,left,base]{\color{textcolor}\rmfamily\fontsize{20.000000}{24.000000}\selectfont \(\displaystyle 0.4\)} 
\end{pgfscope} 
\begin{pgfscope} 
\pgfsetbuttcap 
\pgfsetroundjoin 
\definecolor{currentfill}{rgb}{0.000000,0.000000,0.000000} 
\pgfsetfillcolor{currentfill} 
\pgfsetlinewidth{0.803000pt} 
\definecolor{currentstroke}{rgb}{0.000000,0.000000,0.000000} 
\pgfsetstrokecolor{currentstroke} 
\pgfsetdash{}{0pt} 
\pgfsys@defobject{currentmarker}{\pgfqpoint{-0.048611in}{0.000000in}}{\pgfqpoint{0.000000in}{0.000000in}}{ 
\pgfpathmoveto{\pgfqpoint{0.000000in}{0.000000in}} 
\pgfpathlineto{\pgfqpoint{-0.048611in}{0.000000in}} 
\pgfusepath{stroke,fill} 
} 
\begin{pgfscope} 
\pgfsys@transformshift{0.800000in}{4.056000in} 
\pgfsys@useobject{currentmarker}{} 
\end{pgfscope} 
\end{pgfscope} 
\begin{pgfscope} 
\definecolor{textcolor}{rgb}{0.000000,0.000000,0.000000} 
\pgfsetstrokecolor{textcolor} 
\pgfsetfillcolor{textcolor} 
\pgftext[x=0.360215in,y=3.955981in,left,base]{\color{textcolor}\rmfamily\fontsize{20.000000}{24.000000}\selectfont \(\displaystyle 0.6\)} 
\end{pgfscope} 
\begin{pgfscope} 
\definecolor{textcolor}{rgb}{0.000000,0.000000,0.000000} 
\pgfsetstrokecolor{textcolor} 
\pgfsetfillcolor{textcolor} 
\pgftext[x=0.304660in,y=2.376000in,,bottom,rotate=90.000000]{\color{textcolor}\rmfamily\fontsize{20.000000}{24.000000}\selectfont Probability density} 
\end{pgfscope} 
\begin{pgfscope} 
\pgfpathrectangle{\pgfqpoint{0.800000in}{0.528000in}}{\pgfqpoint{4.960000in}{3.696000in}} 
\pgfusepath{clip} 
\pgfsetbuttcap 
\pgfsetroundjoin 
\pgfsetlinewidth{1.505625pt} 
\definecolor{currentstroke}{rgb}{0.121569,0.466667,0.705882} 
\pgfsetstrokecolor{currentstroke} 
\pgfsetdash{{5.550000pt}{2.400000pt}}{0.000000pt} 
\pgfpathmoveto{\pgfqpoint{1.025455in}{1.816000in}} 
\pgfpathlineto{\pgfqpoint{1.262774in}{0.696000in}} 
\pgfpathlineto{\pgfqpoint{1.500097in}{0.696000in}} 
\pgfpathlineto{\pgfqpoint{1.737416in}{0.696000in}} 
\pgfpathlineto{\pgfqpoint{1.974736in}{0.696000in}} 
\pgfpathlineto{\pgfqpoint{2.212058in}{0.696000in}} 
\pgfpathlineto{\pgfqpoint{2.449378in}{0.696000in}} 
\pgfpathlineto{\pgfqpoint{2.686698in}{0.696000in}} 
\pgfpathlineto{\pgfqpoint{2.924018in}{0.696000in}} 
\pgfpathlineto{\pgfqpoint{3.161340in}{4.056000in}} 
\pgfpathlineto{\pgfqpoint{3.398660in}{0.696000in}} 
\pgfpathlineto{\pgfqpoint{3.635980in}{0.696000in}} 
\pgfpathlineto{\pgfqpoint{3.873302in}{0.696000in}} 
\pgfpathlineto{\pgfqpoint{4.110622in}{0.696000in}} 
\pgfpathlineto{\pgfqpoint{4.347942in}{0.696000in}} 
\pgfpathlineto{\pgfqpoint{4.585261in}{0.696000in}} 
\pgfpathlineto{\pgfqpoint{4.822584in}{0.696000in}} 
\pgfpathlineto{\pgfqpoint{5.059903in}{0.696000in}} 
\pgfpathlineto{\pgfqpoint{5.297223in}{0.696000in}} 
\pgfpathlineto{\pgfqpoint{5.534545in}{1.816000in}} 
\pgfusepath{stroke} 
\end{pgfscope} 
\begin{pgfscope} 
\pgfsetrectcap 
\pgfsetmiterjoin 
\pgfsetlinewidth{0.803000pt} 
\definecolor{currentstroke}{rgb}{0.000000,0.000000,0.000000} 
\pgfsetstrokecolor{currentstroke} 
\pgfsetdash{}{0pt} 
\pgfpathmoveto{\pgfqpoint{0.800000in}{0.528000in}} 
\pgfpathlineto{\pgfqpoint{0.800000in}{4.224000in}} 
\pgfusepath{stroke} 
\end{pgfscope} 
\begin{pgfscope} 
\pgfsetrectcap 
\pgfsetmiterjoin 
\pgfsetlinewidth{0.803000pt} 
\definecolor{currentstroke}{rgb}{0.000000,0.000000,0.000000} 
\pgfsetstrokecolor{currentstroke} 
\pgfsetdash{}{0pt} 
\pgfpathmoveto{\pgfqpoint{5.760000in}{0.528000in}} 
\pgfpathlineto{\pgfqpoint{5.760000in}{4.224000in}} 
\pgfusepath{stroke} 
\end{pgfscope} 
\begin{pgfscope} 
\pgfsetrectcap 
\pgfsetmiterjoin 
\pgfsetlinewidth{0.803000pt} 
\definecolor{currentstroke}{rgb}{0.000000,0.000000,0.000000} 
\pgfsetstrokecolor{currentstroke} 
\pgfsetdash{}{0pt} 
\pgfpathmoveto{\pgfqpoint{0.800000in}{0.528000in}} 
\pgfpathlineto{\pgfqpoint{5.760000in}{0.528000in}} 
\pgfusepath{stroke} 
\end{pgfscope} 
\begin{pgfscope} 
\pgfsetrectcap 
\pgfsetmiterjoin 
\pgfsetlinewidth{0.803000pt} 
\definecolor{currentstroke}{rgb}{0.000000,0.000000,0.000000} 
\pgfsetstrokecolor{currentstroke} 
\pgfsetdash{}{0pt} 
\pgfpathmoveto{\pgfqpoint{0.800000in}{4.224000in}} 
\pgfpathlineto{\pgfqpoint{5.760000in}{4.224000in}} 
\pgfusepath{stroke} 
\end{pgfscope} 
\end{pgfpicture} 
\makeatother 
\endgroup 


==> images/gammas_semi_supervised.tex <==

\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100} 
\definecolor{mycolor2}{rgb}{0.85000,0.32500,0.09800} 
\definecolor{mycolor3}{rgb}{0.92900,0.69400,0.12500} 
 
\begin{tikzpicture}

\begin{axis}[ 
width=2.8in,
height=0.8in,
at={(0.758in,0.481in)},
scale only axis,
xmin=0,
xmax=50,
xlabel style={font=\color{white!15!black}},
xlabel={epochs},
ymin=-0.2,
ymax=1.2,
ylabel style={font=\color{white!15!black}},
ylabel={val. loss - train. loss},
axis background/.style={fill=white}
]
\addplot [ color=black,
                dash pattern=on 1pt off 3pt on 3pt off 3pt, forget plot]
  table[row sep=crcr]{ 
1	-0.0146\\
2	-0.020491\\
3	-0.03454\\
4	-0.044948\\
5	-0.062871\\
6	-0.052588\\
7	-0.038852\\
8	0.022283\\
9	0.026367\\
10	0.06267\\
11	0.115013\\
12	0.337518\\
13	0.279202\\
14	0.461939\\
15	0.353554\\
16	0.620365\\
17	0.609262\\
18	0.629245\\
19	0.613158\\
20	0.79819\\
21	1.047408\\
22	0.756289\\
23	0.574803\\
24	0.74969\\
25	0.645984\\
26	0.669029\\
27	0.851897\\
28	0.761453\\
29	0.530914\\
30	0.88912\\
31	0.789673\\
32	0.776789\\
33	0.684963\\
34	0.679344\\
35	0.69154\\
36	0.58183\\
37	0.557511\\
38	0.558497\\
39	0.630093\\
40	0.635165\\
41	0.687109\\
42	0.670695\\
43	0.708623\\
44	0.703533\\
45	0.635898\\
46	0.733276\\
47	0.597587\\
48	0.542269\\
49	0.552185\\
50	0.523775\\
};
\addplot [color=black,
                smooth, forget plot]
  table[row sep=crcr]{ 
1	-0.020083\\
2	-0.034828\\
3	-0.041414\\
4	-0.068994\\
5	-0.082315\\
6	-0.084936\\
7	-0.065327\\
8	-0.032903\\
9	0.028245\\
10	0.015418\\
11	0.077941\\
12	0.190544\\
13	0.127146\\
14	0.195211\\
15	0.325694\\
16	0.495453\\
17	0.262646\\
18	0.407664\\
19	0.537773\\
20	0.530011\\
21	0.313609\\
22	0.408531\\
23	0.270102\\
24	0.78842\\
25	0.351807\\
26	0.482898\\
27	0.441483\\
28	0.412448\\
29	0.591506\\
30	0.492576\\
31	0.28587\\
32	0.410771\\
33	0.445066\\
34	0.397029\\
35	0.494835\\
36	0.351631\\
37	0.372128\\
38	0.435879\\
39	0.414524\\
40	0.440662\\
41	0.405002\\
42	0.460846\\
43	0.490234\\
44	0.449108\\
45	0.428192\\
46	0.459276\\
47	0.514107\\
48	0.456163\\
49	0.394698\\
50	0.47609\\
};
\addplot [color=black,
                dotted,
                smooth, forget plot]
  table[row sep=crcr]{ 
1	-0.013997\\
2	-0.021594\\
3	-0.019749\\
4	-0.026452\\
5	-0.017474\\
6	0.015677\\
7	0.016196\\
8	0.028161\\
9	0.065555\\
10	0.130449\\
11	0.150553\\
12	0.216045\\
13	0.263967\\
14	0.355523\\
15	0.358838\\
16	0.38597\\
17	0.422147\\
18	0.265475\\
19	0.536938\\
20	0.275884\\
21	0.860152\\
22	0.311852\\
23	0.392896\\
24	0.647758\\
25	0.641321\\
26	0.39052\\
27	0.357822\\
28	0.549876\\
29	0.481288\\
30	0.626727\\
31	0.37369\\
32	0.436187\\
33	0.408156\\
34	0.380425\\
35	0.553106\\
36	0.411105\\
37	0.426608\\
38	0.415271\\
39	0.519741\\
40	0.344306\\
41	0.333286\\
42	0.478583\\
43	0.406547\\
44	0.468316\\
45	0.433531\\
46	0.410427\\
47	0.406669\\
48	0.451838\\
49	0.440662\\
50	0.315889\\
};
\end{axis}
\end{tikzpicture} 


